Adaptive Private Distributed Matrix Multiplication

We consider the problem of designing codes with flexible rate (referred to as rateless codes), for private distributed matrix-matrix multiplication. A master server owns two private matrices $\mathbf{A}$ and $\mathbf{B}$ and hires worker nodes to help computing their multiplication. The matrices should remain information-theoretically private from the workers. Codes with fixed rate require the master to assign tasks to the workers and then wait for a predetermined number of workers to finish their assigned tasks. The size of the tasks, hence the rate of the scheme, depends on the number of workers that the master waits for. We design a rateless private matrix-matrix multiplication scheme, called RPM3. In contrast to fixed-rate schemes, our scheme fixes the size of the tasks and allows the master to send multiple tasks to the workers. The master keeps sending tasks and receiving results until it can decode the multiplication; rendering the scheme flexible and adaptive to heterogeneous environments. Despite resulting in a smaller rate than known straggler-tolerant schemes, RPM3 provides a smaller mean waiting time of the master by leveraging the heterogeneity of the workers. The waiting time is studied under two different models for the workers' service time. We provide upper bounds for the mean waiting time under both models. In addition, we provide lower bounds on the mean waiting time under the worker-dependent fixed service time model.

==> commented_text.tex <==
%Consider the matrices $A \in \F^{s\times r}$ and $B \in \F^{s\times t}$. Let $C=A^TB$ be the product of interest to who splits the matrices $A$ and $B$ into sub-matrices 
%\bes
% A = \left[A_1,A_2,\dots,A_m\right] \qquad B = \left[B_1,B_2,\dots,B_n\right].
%\ees
%Thus, the computed matrix $C$ can be written as 
%\bes
% C = \bbm A_1^TB_1 & A_1^TB_2 & \dots & A_1^TB_n \\
% 		  A_2^TB_1 & A_2^TB_2 & \dots & A_2^TB_n \\
% 		  \vdots & \vdots &\ddots & \vdots \\
% 		  A_m^TB_1 & A_m^TB_2 & \dots & A_m^TB_n
% \ebm.
%\ees
%The computation is now equivalent to computing $mn$ products $A_i^TB_j$ for $i \in [m]$ and $j \in [n]$. Due to privacy constraints, extra random matrices must be used to ``mask'' the private matrices
%The privacy of $A$ is maintained by encoding $A$ with a random matrix $R$ using some polynomial code. For example, to maintain the privacy of $A\triangleq \bbm A_1, A_2 \ebm$ against $T=1$, i.e., no colluding workers, it is sufficient to encode $A$ and a matrix $R$ as follows using a polynomial $g(x) = A_1 + A_2 x + Rx^2$. Giving one evaluation of $g(x)$ to each worker does not violate the privacy of $A$. A similar technique is used to maintain the privacy of $B$, let $f(x) = B_1+B_2x^3+S x^4$. \rb{Trying to add an example on how privacy and encoding is done.}
%
%Therefore we introduce our \temp{framework} as a concatenation between LT \cite{factored_lt} - and Lagrange coded \cite{yu2018lagrange} computing. Let's denote by $\tilde{A}_i$ (similarly by $\tilde{B}_i$) the packets encoded in a LT manner as described in \cite{factored_lt}. %Then we will construct two Lagrange polynomials $f(x)$ and $g(x)$
%We will assume that at most $T$ workers can communicate with each other and both matrices should be kept private, i.e., any T colluding workers should learn nothing about $A$ and $B$. We will construct two Lagrange polynomial $f(x)$ and $g(x)$ in the following way 
%\bas
%f(x) &= \sum_{\ell \in [d]} \tilde{A}_\ell \prod_{k \in [d+T]\setminus \{\ell\}} \frac{x - \alpha_k}{\alpha_\ell-\alpha_k}  \\
% &+ \sum_{\ell=d+1}^{d+T} R_{\ell-d} \prod_{k \in [d+T]\setminus \{\ell\}} \frac{x - \alpha_k}{\alpha_\ell-\alpha_k} 
%\end{align*}
%where $\alpha_i \in \F$ for $i \in [d+T]$ are some distinct evaluation points and $R_t$'s for $t \in [T]$ are matrices chosen at uniformly random from the field $\F$ and $d$ is the degree of the data part, \temp{chosen randomly while encoding the data in a LT manner}. Similarly, $g(x)$ can be written as 
%\bas
%g(x) &= \sum_{\ell \in [d]} \tilde{B}_\ell \prod_{k \in [d+T]\setminus \{\ell\}} \frac{x - \alpha_k}{\alpha_\ell-\alpha_k}  \\
%&+ \sum_{\ell=d+1}^{d+T} S_{\ell-d} \prod_{k \in [d+T]\setminus \{\ell\}} \frac{x - \alpha_k}{\alpha_\ell-\alpha_k}.
%\end{align*}
%where $S_t$'s for $t \in [T]$ are matrices chosen at uniformly random from the field $\F$. It is important that the same evaluation points are used for both polynomials. The master node should give to a worker $i$, both polynomials evaluated at $a_i$ where the following should hold $a_i \notin \{\alpha_1,\dots,\alpha_d\}$, in order to guarantee privacy. The worker should compute $h(a_i)=f(a_i)g(a_i)$ and then return $h(a_i)$ to the master. \\
%In order to interpolate $h(x)$, the master needs to collect $2d+2T-1$ evaluations and afterwards it can start decoding the LT packets by using $h(\alpha_1),\dots,h(\alpha_d)$ as received symbols and apply peeling \temp{(inactivation)} decoding. 

%The other Lagrange polynomial $g(x)$ is constructed in the same way, with the only difference in replacing the coefficients $\tilde{A}_l$'s with $\tilde{B}_\ell$ and $R_t$'s with $S_t$'s.

 %\subsection{Encoding} Let $\omega(x) = \sum$ 
%%\begin{table*}[t!]
%%\centering
%%\begin{tikzpicture}
%%\definecolor{ceruleanblue}{rgb}{0.16, 0.32, 0.75}
%%\definecolor{darkcandyapplered}{rgb}{0.64, 0.0, 0.0}
%%\definecolor{ogreen}{rgb}{0,0.5,0}
%%\def\ogreen{\color{ogreen} \bf}
%%%\node[businessman,monitor,minimum size=0.6cm,shirt=ceruleanblue, saturated] (b) at (0,0) {} node[below=0 of b,font=\small] {User};
%%%\node[inner sep=0pt, right = 5 cm of b] (s2)  {\includegraphics[width=0.6cm]{s1.png}}node[below=0 of s2, font=\tiny] {Server 2} node[right=0 of s2, fill = blue!50,font=\footnotesize] {$X$};
%%%\node[inner sep=0pt, above = 0.8 cm of s2] (s1)  {\includegraphics[width=0.6cm]{s1.png}} node[below=0 of s1, font=\tiny] {Server 1} node[maninblack,mirrored, %evil ,horns =darkcandyapplered, 
%%%minimum size=0.4cm ,above left= -0.3 and -0.2 of s1]{}  node[right=0 of s1, fill = blue!50,font=\footnotesize] {$X$};
%%%\node[inner sep=0pt, below = 0.8 cm of s2] (s3) {\includegraphics[width=0.6cm]{s1.png}} node[below=0 of s3, font=\tiny] {Server 3} node[right=0 of s3, fill = blue!50,font=\footnotesize] {$X$};
%%%%\begin{table*}[t!]
%%%%\normalsize
%%%
%%%\path[->, thick]
%%%	(b)++(1,0.9) edge node [near end,above,sloped, font=\footnotesize] {${\ogreen r_1},\ {\ogreen r_2}$} (s1) 
%%%	(b)++(1,-0.1) edge node [midway,above=-0.1,sloped, font=\footnotesize] {${\ogreen e_{i_1}+r_1},\ {\ogreen e_{i_2}+r_2}$} (s2)
%%%	(b)++(1,-1.1) edge node [midway,above=-0.1,sloped, font=\footnotesize] {${\ogreen e_{i_2}+r_1},\ {\ogreen e_{i_1}+2r_2}$} (s3);
%%%	
%%%\path[->, thick, dashed]
%%%	(s1.south west) edge node[near end,below=-0.1,sloped,font=\footnotesize] {${\blue r_{1}X},\ r_2X$} (1,0.7)++(b)
%%%	(s2.south west) edge node[midway,below=-0.1,sloped,font=\footnotesize] {${\blue  (e_{i_1}+r_1)X},\ (e_{i_2}+r_2)X$} (1,-0.3)++(b)
%%%	(s3.south west) edge node[midway,below=-0.1,sloped,font=\footnotesize] {${\blue (e_{i_2}+r_1)X},\ (e_{i_1}+2r_2)X$} (1,-1.3);
%%	
%%\node[font = \small] (t) at (0,0) {\centering
%%\renewcommand{\arraystretch}{1.2}
%%\begin{tabular}[h!]{c|c|c|c}
%%~& Server1 & Server 2 & Server 3\\ \hline
%%Storage & $\mathbf{x}$ & $\mathbf{x}$ & $\mathbf{x}$ \\ \hline
%%\multirow{2}{*}{Queries}&   $\mathbf{r}_1$ &  $\mathbf{e}_{i}+\mathbf{r}_1$ &  $2\mathbf{e}_{i}+\mathbf{e}_{m+i}+\mathbf{r}_1$\\
%%~& $\mathbf{r}_2$ &  $\mathbf{e}_{m+i}+\mathbf{r}_2$ & $2\mathbf{e}_{m+i}+\mathbf{r}_2$ \\ \hline
%%\multirow{2}{*}{Responses} & \blue $\mathbf{r}_1^T\mathbf{x}$ & \blue $(\mathbf{e}_{i}+\mathbf{r}_1)^T\mathbf{x}$ & \blue $(2\mathbf{e}_{i}+\mathbf{e}_{m+i}+\mathbf{r}_1)^T\mathbf{x}$\\
%%~& $\mathbf{r}_2^T\mathbf{x}$ &  $(\mathbf{e}_{m+i}+\mathbf{r}_2)^T\mathbf{x}$ & $(2\mathbf{e}_{m+i}+\mathbf{r}_2)^T\mathbf{x}$ \\
%%\end{tabular}
%%};
%%
%%\draw[dashed] (5,2) -- (5,-2);
%%
%%\node[above right =-1 and 0.5 of t] (x) {$\mathbf{x}=\begin{bmatrix} x_1,\dots,x_m, x_{m+1},\dots,x_{2m} \end{bmatrix}^T$};	
%%\node[below=0.2 of x] (f) {$f_i = [x_i,\ x_{m+i}]=[\mathbf{e}_i^T\mathbf{x},\ \mathbf{e}^T_{m+i}\mathbf{x}]$};
%%\node[below = 0.2 of f] (e) {$\mathbf{e}_i= [{0},\dots,0,\underbrace{1}_{\textstyle i^\text{th}},0,\dots,{0}]^T$};
%%\node[below right=-0.4 and -1.6 of e] {entry};
%%\node[below = 0 of e] (r) {$\mathbf{r}_1$ and $\mathbf{r}_2$: random vectors};
%%\node[above=0.3 of x] (n) {\em \large Notation};
%%
%%	
%%\end{tikzpicture}
%%\vspace{0.1cm}
%%%\captionsetup{width=0.95\textwidth}
%%\caption{An example of Staircase-PIR code for $n=3$, $k=2$ and $t=1$. %The database $X$ is replicated on all servers. Each file $i$ of the database is divided into two parts $x_i$ and $x_{m+i}$. 
%%The user sends $2$ sub-queries to each server. Each server projects the data on the sub-query vectors and sends the result to the user. If all $3$ servers are not stragglers, the user only downloads the first response (in blue) from each server to retrieve the required file as follows $x_{i} = (\mathbf{e}_{i}+\mathbf{r}_1)^T\mathbf{x} - \mathbf{r}_1^T\mathbf{x}$ and $x_{m+i} =(2\mathbf{e}_{i}+\mathbf{e}_{m+i}+\mathbf{r}_1)^T\mathbf{x} - \mathbf{r}_1^T\mathbf{x}-2x_{i}$. The rate of this scheme is equal to $C(1,3)=2/3$, because the user downloads $3$ responses to retrieve the $2$ parts of the file $f_i=[x_i,\ x_{m+i}]$. If $1$ server is a straggler, the user downloads $2$ responses from each of the remaining servers to retrieve the file. The user can retrieve the file irrespective of which server is a straggler. The rate of this scheme is $C(1,2)=1/2$, because the user downloads $4$ responses to retrieve the file.}
%%\label{fig:intro}
%%%\end{table*}
%%\vspace{-0.5cm}
%%\end{table*}

%\begin{example}[]
%\label{ex:uni} %
%
%\end{example}
%
%
%
%
%\noindent{\em{Related work:}} 
%
%
%\noindent{\em Contributions:}  
%
%\section{Problem formulation and main results}\label{sec:sys}
%
%\section{General framework}% \label{sec:XX}
%\subsection{Construction} %\label{sec:XX}
%
%\bes
% % \resizebox{0.93\textwidth}{!}{
%\label{eq:matcon}
%  \begin{tikzpicture}[baseline=(current  bounding  box.center)]
%\tikzstyle{stealth} = [draw=none,text=black]
%\node[stealth] (1) at (0,0){$
%\mathcal{M}_1=\hspace{0.3cm} \bbm
%\multirow{2}{*}{$\cf$} \\
%\\
% \ck_1\\
%\ebm$                 };
%
%
%\node[stealth] (2) [right=0.1cm of 1] {and      $\mathcal{M}_j=\hspace{0.3cm}\bbm
%\cd_{j-1} \\ \ck_{j} \\ \mathbf{0} \ebm \quad j\neq 1$,} ;
%
%%%%%%grid
%%\def\xMin{-2};
%%\def\xMax{14};
%%\def\yMin{-2};
%%\def\yMax{2};
%%
%%
%%    \foreach \i in {\xMin,...,\xMax} {
%%        \draw [very thin,gray] (\i,\yMin) -- (\i,\yMax)  node [below] at (\i,\yMin) {$\i$};
%%    }
%%    \foreach \i in {\yMin,...,\yMax} {
%%        \draw [very thin,gray] (\xMin,\i) -- (\xMax,\i) node [left] at (\xMin,\i) {$\i$};
%%    }
%\end{tikzpicture}
%%}
%\vspace{-0.2cm}
%\ees
%
%\begin{table}[h!]
%%\be
%\centering
%\resizebox{!}{0.08\textwidth}{
%\begin{tikzpicture}[baseline=(current  bounding  box.center)]
%\tikzstyle{stealth} = [draw=none,text=black]
%
%%\def\x{-0.035}
%%\draw[draw=none,fill=xgray]  (-0.955+\x,-0.92) -- (-0.955+\x,-0.49) -- (-0.21+\x,-0.49) -- (-.21+\x,-.3) -- (.532+\x,-.3) -- 
%%(.532+\x,0) -- (1.245+\x,0) -- (1.245+\x,0.15) -- (2.38+\x,0.15) -- (2.38+\x,-0.92) -- cycle; 
%
%\node[stealth] at (0,0)
%{$\mathcal{M}=\left[\!
%\begin{array}{c:c:c:c:c} 
% ~ & ~ &\multirow{2}{*}{$\cd_2$}  & \dots & \cd_{h-1}\\
% ~& \multirow{2}{*}{$\cd_1$} & & & \multirow{2}{*}{$\ck_h$} \\
%\multirow{2}{*}{$\mathcal{E}$} & & \multirow{2}{*}{$\ck_3$}  &  \dots  & \\ 
% & \multirow{2}{*}{$\ck_2$} & & & \multirow{3}{*}{$\mathbf{0}$} \\
%\multirow{2}{*}{$\ck_1$} &  & \multirow{2}{*}{$\mathbf{0}$} & \dots & \\
% & \mathbf{0} & & & \\
% \end{array}\!\right].$};
%
%%
%%%%%%grid
%%\def\xMin{-4};
%%\def\xMax{4};
%%\def\yMin{-2};
%%\def\yMax{1.5};
%
%
%%    \foreach \i in {\xMin,...,\xMax} {
%%        \draw [very thin,gray] (\i,\yMin) -- (\i,\yMax)  node [below] at (\i,\yMin) {$\i$};
%%    }
%%    \foreach \i in {\yMin,...,\yMax} {
%%        \draw [very thin,gray] (\xMin,\i) -- (\xMax,\i) node [left] at (\xMin,\i) {$\i$};
%%    }
% \end{tikzpicture}
% }
% %\ee
% \caption{ The structure of the matrix $\mathcal{M}$ used to encode the queries of Staircase-PIR. }
% \label{tab:unim}
%\end{table}

==> ex2_table.tex <==
\begin{table*}[t]
    \centering
    \renewcommand{\arraystretch}{1.2}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{c|c|c|c|c|c}
    Time & Worker~$1$ & Worker~$2$ & Worker~$3$ & Worker~$4$ & Worker~$5$ \\ \hline%
    %
      \tikzmark[xshift=-0.33cm,yshift=0ex]{x}%
      %
      \multirow{2}{*}{$1$} & $\Fdata{A_1}(1-a_1)+R_1 a_1$ &  $\Fdata{A_1}(1-a_2)+R_1 a_2$ &    $\Fdata{A_1}(1-a_3)+R_1 a_3$&  $(\Fdata{A_1+A_2})(1-a_4)+R_1 a_4$&  ($\Fdata{A_1+A_2})(1-a_5)+R_1 a_5$ \\ %
      %
       \tikzmark[xshift=-0.35cm,yshift=-3ex]{y} %
       ~ & $\Fdata{B_1}(1-a_1)+S_1 a_1$ &  $\Fdata{B_1}(1-a_2)+S_1 a_2$ &  $\Fdata{B_1}(1-a_3)+S_1 a_3$&  $\Fdata{B_1}(1-a_4)+S_1 a_4$&   $\Fdata{B_1}(1-a_5)+S_1 a_5$ \\[0.5em] \cline{1-1}\cdashline{5-5}%
       %
       \tikzmark[xshift=-1.5cm,yshift=1ex]{t21}%
       \multirow{2}{*}{$2$} & ~ & ~ & ~ & $\Fdata{A_2}(1-a_1) + R_2a_1$ & ~ \\
       ~ &~ & ~ & ~ & $\Fdata{B_2}(1-a_1) + S_2a_1$ & ~ \\[0.5em] \cline{1-1} \cdashline{3-3} \cdashline{6-6}%
       %
       \multirow{2}{*}{$3$} & ~ & $\Fdata{A_2}(1-a_2) + R_2a_2$ & ~ & ~ & $\Fdata{A_2}(1-a_3) + R_2a_3$ \\
       ~ & ~ & $\Fdata{B_2}(1-a_2) + S_2a_2$ & ~ & ~ & $\Fdata{B_2}(1-a_3) + S_2a_3$ \\[0.5em] \cline{1-1} \cdashline{2-2}\cdashline{5-5}%
       %
      \tikzmark[xshift=-0.3cm,yshift=-4.5ex]{t22}%
      \multirow{2}{*}{$4$} & $\Fdata{A_2}(1-a_4) + R_2a_4$ & ~ &  & $\Fdata{A_2}(1-a_2) + R_3a_2$ & ~ \\ 
       ~& $\Fdata{B_1}(1-a_4) + S_2a_4$ & ~ &  & $(\Fdata{B_1+B_2})(1-a_2) + S_3a_2$ & ~ \\[0.5em] \cline{1-1}\cdashline{3-4}%
       %
     \tikzmark[xshift=-1.5cm,yshift=3ex]{t31}%
     \multirow{2}{*}{$5$} & ~ & $\Fdata{A_2}(1-a_1) + R_3a_1$ & $\Fdata{A_2}(1-a_5) + R_2a_5$ &  & ~ \\
      ~& ~ & $(\Fdata{B_1+B_2})(1-a_1) + S_3a_1$ & $\Fdata{B_1}(1-a_5) + S_2a_5$ &  & ~\\[1em] \cline{1-1}\cdashline{6-6} %
       %
       \multirow{2}{*}{$6$} & ~ & ~ & ~ &~ & $\Fdata{A_2}(1-a_3) + R_3a_3$ \\
      \tikzmark[xshift=-1.5cm,yshift=-1ex]{t32}%
      ~ & ~ & ~ & ~ & ~ & $(\Fdata{B_1+B_2})(1-a_3) + S_3a_3$ %\\[1em]
    \end{tabular}
    }
    
    % \drawbrace[brace mirrored, thick]{x}{y}
    % \drawbrace[brace mirrored, thick]{t21}{t22}
    % \drawbrace[brace mirrored, thick]{t31}{t32}
    % \annote[left = 0.1cm]{brace-1}{$t=1$}
    % \annote[left = 0.1cm]{brace-2}{$t=2$}
    % \annote[left = 0.1cm]{brace-3}{$t=3$}
    \caption{A depiction of the proposed rateless scheme with $N=5$ workers and $T=1$ colluding workers. At time $t=1$, the master generates $\widetilde{A}^{(1)}_1 = A_1$, $\widetilde{A}_1^{(2)} = A_1+A_2$, $\widetilde{B}^{(1)}_1 = \widetilde{B}^{(2)}_1 = B_1$ and two random matrices $R_1$ and $S_1$. The master encodes the generated matrices using the polynomials shown in~\eqref{eq:encoding} and sends an evaluation of $f^{(1)}_1(x)$ and $g^{(1)}_1(x)$ to workers 1,2,3 and an evaluation of $f^{(2)}_1(x)$ and $g^{(2)}_1(x)$ to workers $4$ and $5$. Each worker multiplies the obtained evaluations and sends the result to the master. At time $2$, worker~$4$ finishes its computation. The master generates a new task and sends it to this worker. Since worker $4$ finished a task from round $t=1$, the master generates a new task by setting $t=2$ for that worker (the generated linear combinations of $A$ and $B$ are marked in blue boldface letters). At time $3$, the master does the same for workers $2$ and $5$, and so on. A dashed line marks the end of a round at a given worker. At time $6$, one can verify that the master needs to receive the responses from workers $1$ and $3$ or the responses of workers $2,3$ and $5$ in order to finish the multiplication. Notice that faster workers ($2,3,5$) obtained more tasks than the others. Privacy of the matrices is guaranteed by masking $A$ and $B$ with new random matrices at each round.}
    \label{tab:intro-ex}
\end{table*}

==> motivating_example.tex <==
Assume the master has access to $N = 5$ workers that can help with the computation of $C=AB$. Let $T=1$, i.e., the workers do not collude.
% To maintain privacy, the master generates two random matrices $R$ and $S$ that can ``mask'' the data from the workers. 

% The master chooses four numbers $a_i \neq 0$, $i=1,\dots,4$, and sends to each worker $i$ one evaluation of each polynomial $g(a_i)$ and $f(a_i)$. Each worker computes $h(a_i)\triangleq g(a_i) f(a_i)$ and sends the result to the master. Notice that $h(x)$ is a polynomial of degree $2$, thus given any three evaluations of $h(x)$ the master can decode $h(0)=A^TB$. This scheme allows the master to privately distribute the multiplication of $A^TB$ and tolerates one stragglers. However, if there were no stragglers, the master would still ignore the results of one worker. 

We want a scheme that allows the master to adaptively assign small tasks to the workers such that at the end of the algorithm each worker gets a number of tasks that is proportional to their computational resources.
% tolerate the presence of a straggler and fully utilize the computations at the workers in the case of no stragglers. Moreover, we allow the workers to be partially stragglers, i.e., the workers may compute a part of the assigned tasks to them and send the result to the master.

To that end, the master splits $A$ row-wise and $B$ column-wise into two matrices each, i.e., $A \triangleq \bbm A_1^T, A_2^T \ebm^T$, $B \triangleq \bbm B_1, B_2 \ebm$.
The desired computation becomes%
\begin{equation*}
 C = \bbm A_1B_1 & A_1B_2 \\
 		  A_2B_1 & A_2B_2
 \ebm.    
\end{equation*}
%\awz{I would prefer widetilde over tilde...} \awz{Maybe write $\widetilde{A}_{t}, \widetilde{A}_{t+1},\widetilde{B}_{t}, \widetilde{B}_{t+1}$ here as we have only those four matrices in this example? Right?}
Let $\widetilde{A}_j$ and $\widetilde{B}_l$ \marvin{check for AWZ comment}  be random linear combinations of $A_1$ and $A_2$, and $B_1$ and $B_2$, respectively. The algorithm is time-dependent and divided into rounds. At round $t$, the master creates four packets $\widetilde{A}^{(1)}_{t}$, $\widetilde{A}^{(2)}_{t}$, $\widetilde{B}^{(1)}_{t}$, $\widetilde{B}^{(2)}_{t}$ and two random matrices $R_t$ and $S_t$, and encodes them into four polynomials as follows
\begin{align}\label{eq:encoding}
\begin{aligned}
f^{(1)}_t(x) & = \widetilde{A}_{t}^{(1)} (1-x)+ R_tx, \\ g^{(1)}_t(x) &= \widetilde{B}^{(1)}_{t}(1-x) + S_tx,\\
f^{(2)}_t(x) & = \widetilde{A}_{t}^{(2)}(1-x) + R_tx, \\  g^{(2)}_t(x) &= \widetilde{B}_{t}^{(2)}(1-x) + S_tx.
\end{aligned}
\end{align} 
%\awz{Why not denote $f'_t(x)$ by $f_{t+1}(x)$?}

At round $t = 1$, the master chooses five \temp{distinct elements from the finite field} s.t., $a_i\notin \{0,1\}$, $i=1,\dots, 5$, and sends $f^{(1)}_1(a_i)$ and $g^{(1)}_1(a_i)$ to worker $i$, $i=1,2,3$, and $f^{(2)}_1(a_i)$ and $g^{(2)}_1(a_i)$ to worker $i$ for $i=4,5$. The workers multiply $h^{(1)}_1(a_i)\triangleq f^{(1)}_1(a_i)g^{(1)}_1(a_i)$ or $h^{(2)}_1(a_i)\triangleq f^{(2)}_1(a_i)g^{(2)}(a_i)$. The master generates $f^{(1)}_2(x), g^{(1)}_2(x), f^{(2)}_2(x)$ and $g^{(2)}_2(x).$ When worker $i$ returns $h^{(1)}_1(a_i)$ or $h^{(2)}_1(a_i)$ to the master, the master sends $f^{(1)}_2(a_i)$ and $g^{(1)}_2(a_i)$ or $f^{(2)}_2(a_i)$ and $g^{(2)}_2(a_i)$ to the worker guaranteeing that $3$ evaluations of $h^{(1)}_2(x)$ and two evaluations $h^{(1)}_2(x)$ can be obtained at the end of round $2$.

By receiving three evaluations of $h^{(1)}_1(x)$, the master can decode $h^{(1)}_1(x)$. In particular the master can decode $h^{(1)}_1(0) = \widetilde{A}_{1}\widetilde{B}_{1}$ and $h^{(1)}_1(1) = R_t S_t$. 
\awz{it would help to write explicitly what $h_1(x)$ is}
Notice that $h(1) = h'(1)$. Therefore, by receiving two additional evaluations of $h^{(2)}(x)$, the master can decode $h^{(2)}(x)$.

The master keeps generating new tasks and sending them to the workers until he can decode $AB$. One instance of this algorithm is depicted and explained in Table~\ref{tab:intro-ex}.

==> open_problems.tex <==
% \begin{itemize}
%     \item General formula for the rate of this code? 
%     \item Plot the rates of our code versus GASP and Kakar et al, Equation~\eqref{eq:ratio1}.
%     \item Time analysis: Analyze the expected waiting time at the master under certain special regimes. Characterize the tradeoff between rate and time. 
%     \item If new workers join, is it better to generate new polynomials? Or generate new evaluations of the old polynomial?
%     % \item Numerical stability. Give randomness using Lagrange and then other cluster (maybe only one) receive tasks encoded using Chebyshev polynomials \cite{fahim2019numerically}
%     %\item If no worker is a straggler, is it better to use GASP to save evaluations?
%     \item {Simulations}
%     % \item How optimal is this? \textcolor{gray}{$h(x)$ and $h'(x)$ share $T$ evaluations can they share more and guarantee privacy?}
%  We    % \item Check Chebyshev polynomials
%     \item {Implementations on serverless systems} \textcolor{red}{Not for JSAIT}
% \end{itemize}
